NM-SpMM: Accelerating Matrix Multiplication Using N:M Sparsity with GPGPU

Deep learning demonstrates effectiveness across a wide range of tasks. However, the dense and over-parameterized nature of these models results in significant resource consumption during deployment. In response to this issue, weight pruning, particularly through N:M sparsity matrix multiplication, offers an efficient solution by transforming dense operations into semi-sparse ones. N:M sparsity provides an option for balancing performance and model accuracy, but introduces more complex programming and optimization challenges. To address these issues, we design a systematic top-down performance analysis model for N:M sparsity. Meanwhile, NM-SpMM is proposed as an efficient general N:M sparsity implementation. Based on our performance analysis, NM-SpMM employs a hierarchical blocking mechanism as a general optimization to enhance data locality, while memory access optimization and pipeline design are introduced as sparsity-aware optimization, allowing it to achieve close-to-theoretical peak performance across different sparsity levels. Experimental results show that NM-SpMM is 2.1x faster than nmSPARSE (the state-of-the-art for general N:M sparsity) and 1.4x to 6.3x faster than cuBLAS's dense GEMM operations, closely approaching the theoretical maximum speedup resulting from the reduction in computation due to sparsity. NM-SpMM is open source and publicly available at https://github.com/M-H482/NM-SpMM.

==> listing/v1_naive.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstset{
 	language = C++, breaklines = true, breakindent = 10pt, lineskip={-1pt}, basicstyle = \rmfamily\footnotesize, commentstyle = {\itshape \color[cmyk]{1,0.4,1,0}}, classoffset = 0, keywordstyle = {\bfseries \color[cmyk]{0,1,0,0}}, stringstyle = {\ttfamily \color[rgb]{0,0,1}}, frame = trbl, framesep=5pt, numbers = left, stepnumber = 1, xrightmargin=7pt, xleftmargin=8pt, numberstyle = \tiny, tabsize = 3, captionpos = t, directivestyle={\color{black}},  emph={vld1q_f32, vfmaq_f32}, emphstyle={\color{blue}},
}
\lstset{escapeinside={<@}{@>}}

{\color{blue}
\begin{figure}[t]
\centering
\small
\begin{minipage}[c]{0.5\textwidth}
\begin{lstlisting}[caption = {Naive Implementation for Vector-wise N:M Sparsity.},label = {list:naive_impl}]

__global__ void <@\textbf{NM-SpMM}@>(float A[m][k], float B[w][n], float D[w][q], float C[m][n], int M, int N, int v){
  // Calculate indices of thread's computation   
  i = blockIdx.y * blockDim.y + threadIdx.y;
  j = blockIdx.x * blockDim.x + threadIdx.x;
  // Main loop 
  for(int u=0; u<w; u=u+1){
    C[i][j] += A[i][u*M/N+D[u][j/v]]*B[u][j];
  }
}

\end{lstlisting}
\end{minipage}
\end{figure}
}

%%%%%%%%%%%%%%%%%%%%%%%%%

==> listing/v2_hierarchy.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstset{
 	language = C++, breaklines = true, breakindent = 10pt, lineskip={-1pt}, basicstyle = \rmfamily\footnotesize, commentstyle = {\itshape \color[cmyk]{1,0.4,1,0}}, classoffset = 0, keywordstyle = {\bfseries \color[cmyk]{0,1,0,0}}, stringstyle = {\ttfamily \color[rgb]{0,0,1}}, frame = trbl, framesep=5pt, numbers = left, stepnumber = 1, xrightmargin=7pt, xleftmargin=8pt, numberstyle = \tiny, tabsize = 3, captionpos = t, directivestyle={\color{black}},  emph={vld1q_f32, vfmaq_f32}, emphstyle={\color{blue}},
}
\lstset{escapeinside={<@}{@>}}

{\color{blue}
\begin{figure}[ht]
\centering
\small
\begin{minipage}[c]{0.5\textwidth}
\begin{lstlisting}[caption = {Thread Block-level Tiling Implementation.},label = {list:blocking_SM_functionn}]

__device__ void <@\textbf{SMBlock}@>(float As[k_s][m_s], float Bs[w_s][n_s], float Ds[q_s][w_s], float Ct[m_t][n_t], int w_s, int m_t, int n_t){
  // Allocate register buffer
  float At[m_t], Bt[n_t];      
  // Calculate the offset of WARPBLOCK and REGBlock 
  int ti, tj;
  WARPBlock(ti, tj);
  // thread block loop
  for(int p = 0; p < w_s; p++){
    // Load At,Bt from shared memory to register      
    At=LoadFragByIdx(As, ti, p, Ds);
    Bt=LoadFrag(Bs, tj, p);
    // Calculate the outer product of At and Bt
    RegKernel(At, Bt, Ct, m_t, n_t);
  }
}

__device__ void <@\textbf{WARPBlock}@>(int& ti, int& tj){
  int tid = threadIdx.y*blockDim.x + threadIdx.x;
  int warp_id = tid / warpSize; 
  int lane_id = tid % warpSize; 
  // Arrange the threads in a warp into a 4x8 grid
  ti = warp_id/2 * m_t * 4 + lane_id/8 * m_t;            
  tj = warp_id%2 * n_t * 8 + lane_id%8 * n_t;       
}

__device__ void <@\textbf{RegKernel}@>(float At[m_t], float Bt[n_t], float Ct[m_t][n_t], int m_t, int n_t){
  // Calculate the outer product of At and Bt
  for(int i = 0; i < m_t; i++){
    for(int j = 0; j < n_t; j++){
      Ct[i][j] += At[i] * Bt[j]; 
    }  
  }
}

\end{lstlisting}
\end{minipage}
\end{figure}
}

%%%%%%%%%%%%%%%%%%%%%%%%%
